NeutronStream: A Dynamic GNN Training Framework with Sliding Window for Graph Streams

Existing Graph Neural Network (GNN) training frameworks have been designed to help developers easily create performant GNN implementations. However, most existing GNN frameworks assume that the input graphs are static, but ignore that most real-world graphs are constantly evolving. Though many dynamic GNN models have emerged to learn from evolving graphs, the training process of these dynamic GNNs is dramatically different from traditional GNNs in that it captures both the spatial and temporal dependencies of graph updates. This poses new challenges for designing dynamic GNN training frameworks. First, the traditional batched training method fails to capture real-time structural evolution information. Second, the time-dependent nature makes parallel training hard to design. Third, it lacks system supports for users to efficiently implement dynamic GNNs. In this paper, we present NeutronStream, a framework for training dynamic GNN models. NeutronStream abstracts the input dynamic graph into a chronologically updated stream of events and processes the stream with an optimized sliding window to incrementally capture the spatial-temporal dependencies of events. Furthermore, NeutronStream provides a parallel execution engine to tackle the sequential event processing challenge to achieve high performance. NeutronStream also integrates a built-in graph storage structure that supports dynamic updates and provides a set of easy-to-use APIs that allow users to express their dynamic GNNs. Our experimental results demonstrate that, compared to state-of-the-art dynamic GNN implementations, NeutronStream achieves speedups ranging from 1.48X to 5.87X and an average accuracy improvement of 3.97%.

==> section4_storage.tex <==
\section{Dynamic Graph Storage} \label{sec:Dynamic Strorage}

The complex computation of dynamic GNNs algorithm puts more demands on the storage structure of graph topology and node embedding. As shown in Algorithm \ref{alg:dynamic_train}, the dynamic GNN algorithm needs to frequently update the graph topology and node embedding, including reading and updating in-neighbors or out-neighbors, adding or deleting nodes, and adding or deleting edges. 
Since Dynamic GNNs are trained in event-based batch, we need to save multiple version node embeddings of each node embedding for backward propagation.

Existing dynamic GNN models are developed based on the traditional deep learning frameworks \cite{Pytorch_NIPS_2019, Tensorflow_OSDI_2016, MxNet_arXiv_2015}. However, these frameworks do not provide such a graph data structure for users to use, so these algorithm researchers need to design the structure of graph data and node embedding by themselves, which brings them great challenges and burdens. These data structures implemented by users are usually not general, can only support a small subset of models, and are relatively inefficient. In DyRep \cite{DyRep_ICLR_2019}, both the graph topology and the embedding matrix of vertices are stored using matrices. This implementation based on uncompressed matrices requires a lot of memory, which is not friendly to support large-scale graphs. To save multiple version embeddings, when processing each event, DyRep first creates a new matrix and copies the previous embedding matrix, and then updates the node embeddings on this new matrix. This design causes the embedded values of nodes that have not been updated to be stored in multiple copies, resulting in serious redundant storage. In DyGNN \cite{DyGNN_SIGIR_2020}, graph topology is stored using Row-based List of Lists sparse matrix (LIL matrix), which is a sparse matrix stored in rows. It can quickly get the out-neighbors, but cannot get the in-neighbors. Its node embedding is stored using Pytorch's nn.Embedding, which is a simple lookup table that stores embeddings of a fixed dictionary and size. Pytorch's nn.Embedding supports fast reads and writes, but does not support querying arbitrary versions of embeddings. Because it is highly encapsulated, and it only provides users with the latest version of the embedding, but some algorithms need to query earlier versions such as \cite{}. In addition, none of them supports processing streaming graphs, which requires the number of vertices to be known in advance, and does not support node addition and deletion events. However, the graph should be dynamic and unknown in real scenarios.

Based on the above analysis, we designed a dynamic graph storage structure and a multi-version node embedding storage structure to efficiently support the requirements of various dynamic GNN models and the processing of streaming graphs.

\subsection{Dynamic Graph Topology Storage}
\begin{figure}[t]
  \centering
  \vspace{-0.1in}
  \includegraphics[width=\linewidth]{figures/graph_2.pdf}
  \caption{In-Out-Edge-Separated Indexed
Adjacency Lists}
  \vspace{-0.1in}
  \label{fig:graph}
\end{figure}
%受 RisGraph的启发，我们提出了一种新的动态图存储结构，名为\textit{In-Out-Edge-Separated Indexed Adjacency Lists}，如 \autoref{fig:fig5}所示，它分别存储传入和传出边以更通用，这是因为动态GNN的图消息传播可能来自出边和入边，如DGNN。在 \oursys 中，每个顶点都有两个动态数组来存储传入和传出边，包括传入和传出邻居的顶点 Id、边权重和时间戳。 两个动态数组保证了一个顶点的入边和出边都可以连续访问。为了能够提高细粒度访问的能力，我们使用Hash Table为 有大量出边或入边的顶点 建立了邻居节点到动态数组位置的索引.
Inspired by RisGraph \cite{RISGraph_Sigmod_2021}, we propose a dynamic graph storage structure named \textbf{In-Out-Edge-Separated Indexed Adjacency Lists} as shown in \autoref{fig:graph}. It stores incoming and outgoing edges separately for each node to be more general because some models need to access incoming edges like DyRep \cite{DyRep_ICLR_2019}, and some models need to access outgoing edges like DyGNN \cite{DyGNN_SIGIR_2020}.

Each node has two dynamic arrays to store the incoming and outgoing edges, including destination/source node IDs, edge weights, and timestamps. Tow dynamic arrays ensure that a node's incoming and outgoing edges can be visited continuously.  However, arrays suffer from edge lookups by scanning for fine-grained access. For example, when an event needs to update the timestamp of a specified edge, we need to scan this array sequentially, and the time complexity of this operation is $O(n)$. To accelerate lookups, we maintain Key-Value pairs of $<NeighborId \rightarrow Offset>$ for edges, indicating edge locations in arrays. 

We use Hash Table as the default indexes because our data structure with Hash Table provides an average $O(1)$ time complexity for each fine-grained access. Furthermore, the index does not hurt the analysis performance of traversing all the neighbors of a node, because we can directly access the dynamic array to get the information of all the neighbors without involving the index. The indexes of the structure can directly locate edges without scanning, which is friendly for insertions and deletions of an edge.

% ccy: may need to add the node add/delete description


\subsection{Multi-Version Node Embeddings Storage}
To reduce redundant storage and support querying of arbitrary versions of embeddings, we design a multi-version node embedding storage as shown in \autoref{fig:embedding}.
%为了减少冗余存储，我们每一次只存储更新的节点嵌入,经过多个版本后，。我们提供显示为 \autoref{fig:fig6} 的节点表示存储，它包含三个组件：初始节点嵌入矩阵、更新节点嵌入和计数动态数组。一开始 \oursys将每个节点表示组织成一个初始化的节点嵌入矩阵 $Z^{(0)}$。一个新的顶点嵌入用一个零向量初始化并连接到初始化矩阵$Z$，如嵌入矩阵中的虚线所示。我们可以通过 \textit{Count Dynamic Array} 访问最新的节点嵌入。 我们根据节点更新的数量存储更新的节点表示。 在一批事件处理过程中，\oursys 不会直接覆盖旧的节点嵌入，而是将更新的节点表示存储为 $<index \rightarrow embedding>$ 的键值对。
This storage structure contains three components: \textbf{Initialized Embedding Matrix}, \textbf{Updated Node Embeddings}, and \textbf{Node Version Array}. 

In the beginning, the initial embeddings of all known nodes are organized into an initialized embedding matrix $Z^{(0)}$. When a new node needs to be added, we append the embedding of this node into this matrix. As indicated by the dashed line in $Z^{(0)}$, the initial embedding of node $N$ is appended to the embedding matrix. 
During a batch of event processing, we only store updated node embeddings, which avoids redundant storage. We store embeddings with the same version number together, and each updated embedding is stored in the form of Key-Value pair $<NodeID \rightarrow Embedding>$. To speed up access, we use Hash Table as the default indexes.
\textbf{Node Version Array} records the latest version numbers of all nodes. It is a dynamic array that automatically increases size as nodes increase. Each of its elements is only 8 bits and can be accessed atomically. For example, the latest embedding of node 0 is 0, which means we need to find it in $Z^{(0)}$. The latest embedding of node 2 is 2, so this also means we need to find it in $z^{(2)}$.

Based on this structure, we can quickly access and store the specific node embedding through two indexes, and the time complexity is $O(1)$. For example, if we want to find the embedding of node 2 with version number 1. We first need to get the latest version number of node 2 according to the node ID in the dynamic array. The version number is 2, which means that there is an embedding with version number 1. Then we can locate the embedding in $Z^{(1)}$ according to the node ID. The multi-version node embedding storage can support efficient access and modification, avoid redundant storage and provide users with more flexibility.   


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/embedding_2.pdf}
  \caption{Multi-Version Node Embedding Storage}
  \label{fig:embedding}
\end{figure}
